Stochastic Models for Speciation Events in Phylogenetic trees

In a phylogenetic tree, we often don't have information about the time a speciation event (inner node) occured. Under a neutral model for speciation, I develop fast algorithms for calculating the probability that an inner node i is the k-th speciation event. For the Yule and the coalescent model, I develop an edge length estimation as well. Various properties of the Yule model are discussed throughout the thesis.

==> rankprob.tex <==
\noindent
Tanja Gernhard \\
22.02.2006 \\
\\
\\

\noindent
%\begin{algorithm} %[h!]
      %\begin{alg}
        {\bf Algorithm}: \textsc{RankProb}($\cT,v$)  \index{algorithm R\textsc{ankProb}}\\
        {\bf Input}: A rooted binary phylogenetic tree $\cT$ and an interior vertex $v$.\\
        {\bf Output}: The probabilitiess $\bP[r(v)=i]$ for ${i=1, \ldots ,|\Vr|}$.
        \begin{algorithmic}[1]
          \STATE Denote the vertices of the path from $v$ to root $\rho$ with \\ $(v=x_1, x_2, \ldots ,x_n=\rho)$.
          \STATE Denote the subtree of $\cT$, consisting of root $x_m$ and all its descendants, by $\cT_m$ for $m=1, \ldots ,n$.
          \FOR{$m=1, \ldots ,n$}
            \FOR{$i=1, \ldots , |\Vr_{\cT}|$}
                \STATE $\alpha_{\cT_m,v}(i):=0$
            \ENDFOR
          \ENDFOR
          \STATE $\alpha_{\cT_1,v}(1):=1$
          \FOR{$m = 2, \ldots ,n$}      %LINE 9 mentioned in Compare!!!!
            %\STATE $\cT_{m-1}':=\cT_m \setminus (\cT_{m-1}\cup x_m)$ \qquad ({\it cf.} Figure \ref{FigRankCount2})
            \STATE $\cT_{m-1}':=\cT_m | (\sL_{\cT_m} \setminus \sL_{\cT_{m-1}})$ \ref{FigRankCount2})
            \FOR{$i=m, \ldots ,|\Vr_{\cT_m}|$}
                \STATE $M := \min\{|\Vr_{\cT_{m-1}'}|, i-2\}$
                \STATE $\displaystyle \alpha_{\cT_m,v}(i):=$ \\ \quad $\sum_{j=0}^{M} \alpha_{\cT_{m-1},v} (i-j-1)
                {|\Vr_{\cT_{m-1}}|+|\Vr_{\cT_{m-1}'}|-(i-1) \choose |\Vr_{\cT_{m-1}'}|-j} {i-2 \choose j}$
            \ENDFOR
          \ENDFOR
          \FOR{$i=1, \ldots , |\Vr_{\cT}|$}
          	\STATE $\bP[r(v)=i] = \frac{\alpha_{\cT_n,v}(i)}{\sum_{j} \alpha_{\cT_n,v}(j)}$
          \ENDFOR
        \end{algorithmic}
        \bigskip
      %\end{alg}
%\end{algorithm}

